Symbol Rate-Code Rate Trade-offs for IM/DD 200G/400G per Lane LPO Transceivers

We analyze the symbol rate-code rate trade-off in bandwidth-limited IM/DD systems targeting LPO transceivers, using PAM-4/6/8 as candidate modulation formats. We use the capacity of the binary symmetric channel as an achievable information rate under hard-decision decoding, serving as a performance metric for 200G and 400G per-lane throughput targets. Our results show that reducing the FEC code rate below the KP4 baseline allows higher-order PAM formats to operate at substantially lower symbol rates than PAM-4 while meeting the throughput requirement.

==> Figures/schemes/E2E_module_diagram_horizontal.tex <==
\begin{tikzpicture}[
    line width = 1pt,
    every node/.style = {
        node distance = 2em,
        minimum width = 2em,
        minimum height = 2em
    },
    block/.style = {
        draw = RoyalBlue,
        text = RoyalBlue,
        shading = axis,
        top color = RoyalBlue!20!white,
        bottom color = RoyalBlue!5!white,
        rectangle, rounded corners, minimum width=1.1cm, minimum height=1cm, align=center, font=\large
    },
     highlightTRX/.style = {
         rounded corners,
         draw = none,
         text = Plum,
         shading = axis,
         top color =  RoyalBlue!40!white,
         bottom color =  RoyalBlue!8!white,
     },
    redblock/.style = {
        draw = red,
        text = red,
        shading = axis,
        top color = red!20!white,
        bottom color = red!5!white,
        rectangle, rounded corners,
        minimum width=1.55cm,
        minimum height=0.9cm,
        align=center,
        font=\large
    },
    grayblock/.style = {
        draw = gray,
        text = gray,
        shading = axis,
        top color = gray!20!white,
        bottom color = gray!5!white,
        rectangle, rounded corners,
        minimum width=1.55cm,
        minimum height=0.9cm,
        align=center,
        font=\large
    },
    purpleblock/.style = {
        draw = violet,
        text = violet,
        shading = axis,
        top color = violet!20!white,
        bottom color = violet!5!white,
        rectangle, rounded corners,
        minimum width=1.1cm,
        minimum height=1cm,
        align=center,
        font=\large
    },
    orangeblock/.style = {
        draw = orange!80!black,
        text = orange!80!black,
        shading = axis,
        top color = orange!20!white,
        bottom color = orange!5!white,
        rectangle, rounded corners,
        minimum width=1.1cm,
        minimum height=1cm,
        align=center,
        font=\large
    },
    greenblock/.style = {
        draw = ForestGreen,
        text = ForestGreen,
        shading = axis,
        top color = ForestGreen!20!white,
        bottom color = ForestGreen!5!white,
        rectangle, rounded corners,
        minimum width=1.1cm,
        minimum height=1cm,
        align=center,
        font=\large
    },
    ellipseblock/.style={circle, draw = RoyalBlue, fill = white, text = RoyalBlue, minimum size=0.5cm, font=\footnotesize},
    addition/.style={circle, draw = RoyalBlue, fill = white,scale=0.8, text = RoyalBlue, minimum size=0.5cm, font=\footnotesize},
    amp/.style={draw = RoyalBlue, isosceles triangle, isosceles triangle apex angle=60, fill=white, 
    minimum height=1cm, minimum width=1cm, rotate=0, anchor=center},
    amp1/.style={draw = RoyalBlue, isosceles triangle, isosceles triangle apex angle=60, fill=white, 
    minimum height=1cm, minimum width=1cm, rotate=180, anchor=center},
    arrow/.style={-{Stealth[scale=1]}, thick, draw = RoyalBlue},
    backgroundBlockRed/.style={draw = red,
    text = red,
    shading = axis,
    top color = red!20!white,
    bottom color = red!5!white,, rounded corners, minimum width=6cm, minimum height=2.5cm},
    backgroundBlock/.style={draw = RoyalBlue!40!black, fill = RoyalBlue!5, rounded corners, minimum width=6cm, minimum height=2.5cm},
    highlight/.style = {
        rounded corners,
        draw = none,
        text = Plum,
        shading = axis,
        top color = red!40!white,
        bottom color = red!8!white
    }
]



\node[purpleblock, scale=0.9, align=center,minimum width=1.78cm,rotate=0] (preeq) {DAC};
% \node[ redblock, above=0.05em of preeq, align=center] (pshape) {Pulse\\ Shaping};
\node[ redblock, above=0.05em of preeq, align=center] (Mod) {PAM-$M$};
% \draw [redblock] (preeq.north west) rectangle node[anchor = center, name = test] {Test} 

 \node[text = red, above =2.7em of preeq.north , align = center] (Diversity1) {{TRX-DSP}};
\begin{scope}[on background layer]
\draw[highlight] ($(Diversity1.north west) + (-0.01,-0.61)$) rectangle ($(Diversity1.east |- preeq.south) + (0.07, .5)$);
\end{scope}


\draw[->, arrow] ($(Mod.west)+(-0.7,0)$) -- ($(Mod.west)+(0,0)$) node[midway,above] {\large $\boldsymbol{b}$};

% \draw[->, arrow] (PF.east) -- (AMP.west);
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%TX_FON%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    % PCB trace
    \node[block, right=2em of preeq,draw=RoyalBlue] (PCB) {TRF};

    % Amplifier addition
    \node[addition, right=1em of PCB] (add1) {\large $+$};

     %(1-alpha) noise control 
    
    % \node[addition, below=1em of add1] (n_control_1) {\large $\times$};
    % Normalization
    % \node[addition, right=1em of PCB,scale=0.7] (norm) {\large $\mathbf{Norm}$};

     % Amplifier addition
    % \node[addition, right=1em of add1] (addXT) {\large $+$};
    %[xshift=-2.cm, yshift=-0.5cm]EO.center)
    
    \node[block, right=1em of add1,draw=RoyalBlue] (PF) {Peaking \\ Filter};

    % Amplifier addition
    \node[addition, right=1em of PF] (AMP) {\large $+$};



     \node[greenblock, right=0.1em of AMP,   minimum height=1.15cm,draw=ForestGreen] (IM) at ($(AMP.east)+(1.6em,0)$) {\large MZM};

    % RIN
    % \node[block, above=0.5cm of IM, draw=RoyalBlue, dashed] (RIN) {RIN};
    \node[greenblock, above=0.5cm of IM, xshift=-3.2em, yshift=-0.04em,minimum width=2.9cm,  minimum height=1.15cm,dashed,draw=ForestGreen] (RIN) {};

        % thermal noise addition
    \node[addition, above=1.5em of IM, draw = ForestGreen] (Nrin) {\large $+$};

    % helper coords so the highlight can include the wires too
    \coordinate (rin_in)  at ($(Nrin.west)+(-0.8,0)$);
    \coordinate (rin_top) at ($(Nrin.north)+(0,0.3)$);
    \coordinate (rin_topL) at ($(Nrin.north)+(-0.8,0.3)$);
    
    % connections
 \draw[->, arrow,ForestGreen] (rin_in) -- (Nrin.west)
  node[pos=0, below=0pt, xshift=-0.95em, yshift=1.1em,black] {\large ${I}_{\mathrm{0}}$};

    
    \draw[-,ForestGreen] (rin_topL) -- (rin_top) node[pos=0, above=0pt, xshift=-2.75em, yshift=-1.25em,black] {\large $I_{\mathrm{0}}\!\cdot\! n_{\mathrm{RIN}}(t)$};
    \draw[arrow,ForestGreen]     (rin_top)  -- (Nrin.north);


     \node[text = ForestGreen, above =0.01em of Nrin.north , xshift=-6.95em, yshift=-0.1em, align = center,rotate=90,scale=1.12
     ] (DRIN) {\large Laser};
    % \begin{scope}[on background layer]
    

  
    % \node[greenBlock, below=0.8cm of PF, draw=blue] (noise) {$\frac{N_0}{2}$};
    
    % Connections
    \draw[->, arrow] (PCB.east) -- (add1.west);
    % \draw[->,arrow]    (noise.west) -|(n_control_1.south);

    % \draw[->,arrow]    (n_control_1.north) --(add1.south);


    % \draw[->,arrow]   (n_control_2.north) --(AMP.south);
    \draw[->, arrow] (add1.east) -- (PF.west);
    % \draw[->, arrow] (addXT.east) -- (PF.west);
    \draw[->, arrow] (PF.east) -- (AMP.west);
    % \draw[->, arrow] (PF.east) -- (add.west);
    % %\draw[->, arrow] (norm.east) -- (add.west);
    % \draw[->, arrow] (add.east) -- (AMP.west);
    \draw[->, arrow] (AMP.east) -- (IM.west)node[midway,above] {\large $u(t)$};
    % \draw[->, arrow] (add.east) -- (IM.west);
    %\draw[->, arrow] (add.east) -- (BTF.west);
    % \draw[->, arrow] (BTF.east) -- (IM.west);
    \draw[->, arrow,ForestGreen] (Nrin.south) -- (IM.north);

    % \draw[->, arrow] ($(AMP.north)+(0,0.6)$) -- ($(AMP.north)$) node[midway,left] {$n_{\text{in}}$};




    % \draw[->, arrow] ($(n_control_1.west)+(-0.4,0)$) -- ($(n_control_1.west)$) node[midway,left] {$\sqrt{(1-\alpha)}$};


    \draw[->, arrow] ($(add1.south)+(0,-0.6)$) -- ($(add1.south)$) node[midway,left] {\large $n_{XT}(t)$};


    \draw[->, arrow] ($(AMP.south)+(0,-0.6)$) -- ($(AMP.south)$) node[midway,left] {\large $n_{1}(t)$};
    % \draw[->, arrow] ($(n_control_2.east)+(0.4,0)$) -- ($(n_control_2.east)$) node[midway,right] {$\sqrt{\alpha}$};

    % \draw[->, arrow] ($(n_control_2.south)+(0,-0.6)$) -- ($(n_control_2.south)$) node[midway,left] {$n_{1}(t)$};

    
   % \draw[->, arrow] ($(add.north)+(0,0.6)$) -- ($(add.north)$) node[midway,right] {$G$};

    % \draw[->, arrow] ($(addXT.north)+(0,0.6)$) -- ($(addXT.north)$) node[midway,left] {$n_{\text{XT}}(t)$};
    % Inputs and outputs
    % \node[left=0.5cm of PCB] (input) {$\boldsymbol{s}_{\text{up}}(t)$};
    \draw[->, arrow] (preeq.east) -- (PCB.west)node[midway,above]{};% {$\boldsymbol{s}_{\text{u}}(t)$};
    

    
    % \draw[->, arrow] (IM.east) -- (output.west);



    
  % Reference node (stays put and keeps your rectangle math unchanged)
\node[above=3em of PF.south east] (Diversity) {};

% Title node (shifted left, doesn't affect the block geometry)
\node[text=RoyalBlue, align=center, anchor=south] 
  at ($(Diversity.north)+(-7em,0)$) {TRX-Frontend};
    \begin{scope}[on background layer]
    \draw[highlightTRX] ($(Diversity.north west) + (-3.8,1.1)$) rectangle ($(Diversity.east |- AMP.south) + (2.55, -0.8)$);
    \end{scope}


    %%%%%%%%%%%%%%%%%%%%%%% channel %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




     %%%%%%%%%%%%%%%%%%%%%%% receiver frontend  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



     
    \node[addition, right=9em of IM,scale=0.95,draw=ForestGreen] (normRX) {\large$||.||^2$};

    % butterwort filter
    \node[block, right=1em of normRX,draw=RoyalBlue] (PCB_RX) {Butterw. \\ Filter};

    % shot noise addition
    \node[addition, right=1em of PCB_RX] (add_RX) {\large $+$};
    % Normalization

    % Peaking Filter
    \node[block, right=1em of add_RX,draw=RoyalBlue] (PF_RX) {Peaking \\ Filter};

    % thermal noise addition
    \node[addition, right=1em of PF_RX] (TN) {\large $+$};

    % Linear Filtering
    \node[block, right=1em of TN,draw=RoyalBlue] (LF_RX) {TRF};



    \draw[->, arrow] (normRX.east) -- (PCB_RX.west);
    \draw[->, arrow] (PCB_RX.east) -- (add_RX.west);
    \draw[->, arrow] (add_RX.east) -- (PF_RX.west);
    \draw[->, arrow] (PF_RX.east) -- (TN.west);
    \draw[->, arrow] (TN.east) -- (LF_RX.west);

     \draw[->, arrow] ($(TN.south)+(0,-0.8)$) -- ($(TN.south)$) node[midway,left] {\large $n_{\text{T}}(t)$};
    \draw[->, arrow] ($(add_RX.south)+(0,-0.8)$) -- ($(add_RX.south)+(0,0)$) node[midway,left] {\large $n_{\text{S}}(t)$};   

    % Draw the first horizontal segment and label
    % Original horizontal line + label
    \draw[-, ForestGreen]   ($(IM.east)+(0.0,0)$) 
                       -- ($(IM.east)+(0.99,0)$) 
                       node[midway, above, ForestGreen] {\large $E_{\text{Tx}}(t)$};
    
    % Ellipses over the fiber segment
    % Rising ellipses over the arrow path to simulate fiber
    % Ellipses over the fiber segment
    \foreach \x in {1.35,1.45,1.55,1.65,1.75} {
        \node[ellipse, draw=ForestGreen, fill=ForestGreen!1, minimum width=0.4cm, minimum height=0.4cm,opacity=0.6] 
            at ($(IM.east)+(\x, 0.2)$) {};
    }
    
    % Arrow continues from the last ellipse to normRX
    \draw[->, arrow,ForestGreen]   ($(IM.east)+(0.7,0)$) 
                   -- ($(normRX.west)+(0,0)$) node[midway, above, below=-20pt, xshift=2.em, yshift=1, Green] {\large $E_{\text{Rx}}(t)$};;

    
     \node[text = RoyalBlue, below =1.3em of PF_RX.south, align = center] (Diversity2) {RX-Frontend};
    \begin{scope}[on background layer]
    \draw[highlightTRX] ($(Diversity2.north west) + (-4.1,2.5)$) rectangle ($(Diversity2.east |- PF_RX.south) + (2.3, -1.2)$);
    \end{scope}

     \node[above=2.5em of PCB_RX] (ele) {\large Electrical:};

    % simple arrow to the right of the label
    \draw[-{Latex[length=2mm]},RoyalBlue] (ele.east) -- ++(0.65,0);
    
    \node[right=2em of ele] (opt) {\large Optical:};
    \draw[-{Latex[length=2mm]},ForestGreen] (opt.east) -- ++(0.65,0);
    %%%%%%%%%%%%%%%%%%%%%%% receiver DSP %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    %%%%%%%%%%%%%%%%%%%%%%% receiver DSP %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Inverse precoding block
\node[purpleblock, right=2em of LF_RX, yshift=-3.4em,minimum width=1.85cm] (Invprecod) {ADC};
\node[redblock, above=0.01em of Invprecod, yshift=0em,minimum width=1.85cm] (Eq) {FFE};
\node[redblock, above=0.01em of Eq, yshift=0em,minimum width=1.85cm] (MLSE) {MLSE};
\node[redblock, above=0.01em of MLSE,minimum width=1.85cm] (Demod) {Demapper};

% % Demodulator block
% \node[redblock, left=1.5em of Invprecod] (Demod) {Demodulator};

% Connections
\draw[-,RoyalBlue] ($(LF_RX.east)+(0,0)$)-- ($(LF_RX.east)+(0.4,0)$);
\draw[->, arrow] ($(LF_RX.east)+(0.4,0)$)|- ($(Invprecod.west)+(0,0)$);



    


    \draw[->, arrow] ($(Demod.east)+(0,0)$) -- ($(Demod.east)+(0.7,0)$) node[midway,above] {\large $\hat{\boldsymbol{b}}$};

    \node[text = red, above =11em of Invprecod.south, align = center] (Diversity3) {RX-DSP};
    \begin{scope}[on background layer]
    \draw[highlight] ($(Diversity3.north west) + (-0.28,-3.9)$) rectangle ($(Diversity3.east |- PF_RX.south) + (0.29, 2.8)$);
    \end{scope}

% \begin{scope}[on background layer]
%     \filldraw[gray, dashed, thick, rounded corners, fill=gray, fill opacity=0.2] 
%         ($(DFE.north west) + (-0.15,0.25)$) rectangle 
%         ($(MLSE.south east) + (0.25,-0.15)$);
% \end{scope}
\node [font=\Large,anchor=north west] at (9,2) {\shortstack[l]{\textbf{(a)}}};
    
\end{tikzpicture}
